System-Level Analysis of Full-Duplex Self-Backhauled Millimeter Wave Networks

Integrated access and backhaul (IAB) facilitates cost-effective deployment of millimeter wave(mmWave) cellular networks through multihop self-backhauling. Full-duplex (FD) technology, particularly for mmWave systems, is a potential means to overcome latency and throughput challenges faced by IAB networks. We derive practical and tractable throughput and latency constraints using queueing theory and formulate a network utility maximization problem to evaluate both FD-IAB and half-duplex(HD)-IAB networks. We use this to characterize the network-level improvements seen when upgrading from conventional HD IAB nodes to FD ones by deriving closed-form expressions for (i) latency gain of FD-IAB over HD-IAB and (ii) the maximum number of hops that a HD- and FD-IAB network can support while satisfying latency and throughput targets. Extensive simulations illustrate that FD-IAB can facilitate reduced latency, higher throughput, deeper networks, and fairer service. Compared to HD-IAB,FD-IAB can improve throughput by 8x and reduce latency by 4x for a fourth-hop user. In fact, upgrading IAB nodes with FD capability can allow the network to support latency and throughput targets that its HD counterpart fundamentally cannot meet. The gains are more profound for users further from the donor and can be achieved even when residual self-interference is significantly above the noise floor.

==> IEEEtran/IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> IEEEtran/IEEEtran/tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> v2/eq_dump.tex <==
\begin{align}
\label{eq:sum_delay_CDF}
    \bbP\left[D_m \leq d\right] &= \left[\prod_{(u,v)\in \sfR(s,d)}(c_{u,v}\mu_{u,v} - (\bF\blam)_v)\right]\\
    &\times\sum_{(q,r)\in \sfR(s,d)}\frac{e^{-(c_{q,r}\mu_{q,r} - (\bF\blam)_{r})d}}{\prod_{(t,w)\in\sfR(s,d), (t,w)\neq(q,r)}((c_{t,w}\mu_{t,w} - (\bF\blam)_{w}) - (c_{q,r}\mu_{q,r} - (\bF\blam)_{r}))}.
\end{align}

\begin{subequations} \label{opt:per_link}
\begin{align}
\underset{\blam, \bmu}{\textrm{maximize}} ~0\\
\st\nonumber \\
& \blam \geq\bm{0},~\bmu \geq \bm{0},~\bmu \leq \bm{1} \label{opt:per_link_var_intervals}\\
& \bC\bmu - \bm{\ell} > \bm{0} \label{opt:per_link_rate_feas_cons}\\ 
& \bG\bmu\leq \bm{1} \label{opt:per_link_resource_cons}\\
& 1 - e^{-(c_{uv} - \ell_v)\delta/h_m} \geq \eta \quad m = 1, 2, \cdots, M \label{opt:per_link_delay_cons}.
\end{align}
\end{subequations}

We want to find the minimum value of $\delta$ which is feasible for the given network topology. Mathematically,

\begin{subequations} \label{opt:delay_feas_lp}
\begin{align}
\underset{\delta, \bmu}{\textrm{minimize}} ~&\delta\\
\st\nonumber \\
& \blam \geq\bm{0},~\bmu \geq \bm{0},~\bmu \leq \bm{1} \label{opt:delay_feas_lp_var_intervals}\\
& \bC\bmu - \bm{\ell} > \bm{0} \label{opt:delay_feas_lp_rate_feas_cons}\\ 
& \bG\bmu \leq \bm{1} \label{opt:delay_feas_lp_resource_cons}\\
& 1 - e^{-(c_{uv} - \ell_v)\delta/h_m} \geq \eta \quad m = 1, 2, \cdots, M \label{opt:delay_feas_lp_delay_cons}.
\end{align}
\end{subequations}

The above linear program can be reformulated as below. Note that the constraints have been modified so that the delay constraint is large enough so that each UE is guaranteed a minimum arrival rate $\minlam$. This is to avoid degenerate solutions, for example, where $\delta$ is feasible because a minuscule arrival rate can be supported at the the first hop and no other UEs.
\begin{subequations} \label{opt:delay_feas_lp_reform}
\begin{align}
\underset{t, \blam, \bmu}{\textrm{maximize}} ~&t\\
\st\nonumber \\
& \blam \geq\minlam\bm{1},~\bmu \geq \bm{0},~\bmu \leq \bm{1} \label{opt:delay_feas_lp_reform_var_intervals}\\
& \bC\bmu - \bF\blam > t\bh \label{opt:delay_feas_lp_reform_rate_feas_cons}\\ 
& \bG\bmu \leq \bm{1} \label{opt:delay_feas_lp_reform_resource_cons}
\end{align}
\end{subequations}
The feasibility problem in \eqref{opt:delay_feas_lp_reform} is a linear program and can be solved very fast. A network operator could even solve it in real-time as network metrics are reported. The network can adapt its parameters in real-time. 

\begin{lemma}\label{lem:min_lam_opt}
$\minlam\bm{1}$ is an optimal arrival rate vector for \eqref{opt:delay_feas_lp_reform}.
    \begin{proof}
    The proof is by contradiction. Let $\blam^*$ be the optimal arrival rate vector for \eqref{opt:delay_feas_lp_reform} such that $\lambda^*_m > \minlam$ for some $m$. This means there exists at least one $l$ such that $(\bC\bmu - \minlam\bF\bm{1})_l > (\bC\bmu - \bF\blam^*)_l$. If $(\bC\bmu - \bF\blam^*)_l = t^*h_l$, then $\minlam\bm{1}$ achieves a higher objective value than $\blam^*$ and hence is not optimal and we have a contradiction. On the other hand, if $(\bC\bmu - \bF\blam^*)_l > t^*h_l$, then choosing $\minlam\bm{1}$ is also a feasible point that achieves the same objective value.
    \end{proof}
\end{lemma}

\begin{lemma}
Network can support $\minlam$ if \red{Closed-form result in Mandar's work}
\begin{align}
    \bG\bC^{-1}\bF\bm{1}\minlam \leq \bm{1}
\end{align}
\end{lemma}
\begin{lemma}\label{lem:feasible_delay_sol_general}
The solution for \eqref{opt:delay_feas_lp_reform} is given by
\begin{align}
    t^* = \underset{l=1,2,\cdots,K}{\min}\frac{1 - \minlam\bG_k\bC^{-1}\bF\bm{1}}{\bG_k\bC^{-1}\bh} \quad \forall k.
\end{align}
The minimum feasible delay $\delta^*$ is then given by $\delta^* = -\log(1-\eta)/t^*$.
\end{lemma}

\begin{theorem}
If $\cT$ is linear with depth $K$, all edges in $\cT$ have capacity $R$ and $\bC = R\bI$ then 

\begin{align}
    t^*_{\textrm{HD}} = 
     \begin{cases}
        \frac{(1 - 4\minlam/R)R}{3K-1}, ~ \frac{\minlam}{R} \leq \frac{1}{6K + 2} \\
        \frac{(1 - 2(K-1)\minlam/R)R}{2 (K+1)}, ~ \frac{1}{6K + 2} < \frac{\minlam}{R}
    \end{cases}
\end{align}

\begin{align}
    t^*_{\textrm{FD}} = 
     \begin{cases}
        \frac{(1 - 2\minlam/R)R}{2K-1}, ~ \frac{\minlam}{R} \leq \frac{1}{2K + 1} \\
        \frac{(1 - K\minlam/R)R}{K+1}, ~ \frac{\minlam}{R} > \frac{1}{2K + 1}
    \end{cases}
\end{align}
And $\delta^* = \frac{-\log(1 - \eta)}{t^*}$.
\end{theorem}

\begin{lemma}
If $\cT$ is linear with depth $K$, all edges in $\cT$ have capacity $R$ and $\bC = R\bI$ then \red{$(\minlam/R < 1/2)$}.
\begin{align}
    \frac{\delta^*_{\textrm{HD}}}{\delta^*_{\textrm{FD}}} = 
    \begin{cases}
        \frac{(1 - 2\minlam/R)/(2K-1)}{(1 - 4\minlam/R)/(3K-1)}, ~ \frac{\minlam}{R} \leq \frac{1}{6K + 2} \\
        \frac{(1 - 2\minlam/R)/(2K-1)}{(1 - 2(K-1)\minlam/R)/(2K+2)}, ~ \frac{1}{6K + 2} < \frac{\minlam}{R} \leq \frac{1}{2K+1} \\
        \frac{2(1 - K\minlam/R)}{1 - 2(K-1)\minlam/R}, ~ \frac{\minlam}{R} > \frac{1}{2K+1}
    \end{cases}
\end{align}
    \begin{proof}
    For the donor node, $k=0$, $t\leq \frac{(1 - K\minlam/R)R}{K+1}$. For HD and $1\leq k <K-1$, $t\leq \frac{(1 - 2(K-k)\minlam/R)R}{2K+k+1}$. For FD and $1\leq k <K-1$, $t\leq \frac{(1 - (K-k)\minlam/R)R}{K+k+1}$. For $k=K-1$ and HD, $t \leq \frac{(1-2\minlam/R)R}{2K}$. For $k=K-1$ and FD, $t \leq \frac{(1 - \minlam/R)R}{K}$.
    \begin{itemize}
        \item \textit{Case 1}: If $\minlam / R \leq 1/(6K+2)$ then $\frac{(1-2\minlam/R)R}{2K} > \frac{(1 - K\minlam/R)R}{K+1} > \frac{(1 - 2(K-1)\minlam/R)R}{2K+1+1}$ and $\frac{(1 - 2(K-k)\minlam/R)R}{2K+k+1}$ is a decreasing function in $k$. Thus, for half-duplex $t^*_{\textrm{HD}} = \frac{(1 - 2\minlam/R)R}{3K}$. For FD, $\frac{(1-\minlam/R)R}{K} > \frac{(1 - K\minlam/R)R}{K+1} > \frac{(1 - (K-1)\minlam/R)R}{K+1+1}$ and $\frac{(1 - (K-k)\minlam/R)R}{K+k+1}$ is decreasing in $k$. Thus, for FD $t^*_{\textrm{FD}} = \frac{(1 - \minlam/R)R}{2K}$. $\frac{\delta^*_{\textrm{HD}}}{\delta^*_{\textrm{FD}}} = \frac{t^*_{\textrm{FD}}}{t^*_{\textrm{HD}}}$.
        
        \item \textit{Case 2}: If $\frac{1}{6K + 2} < \frac{\minlam}{R} \leq \frac{1}{2K+1}$  then $\frac{(1-2\minlam/R)R}{2K} > \frac{(1 - K\minlam/R)R}{K+1} > \frac{(1 - 2(K-1)\minlam/R)R}{2K+1+1}$ and $\frac{(1 - 2(K-k)\minlam/R)R}{2K+k+1}$ is a increasing function in $k$. Thus, for half-duplex $t^*_{\textrm{HD}} = \frac{(1 - 2(K-1)\minlam/R)R}{2(K+2)}$. For FD, $\frac{(1-\minlam/R)R}{K} > \frac{(1 - K\minlam/R)R}{K+1} > \frac{(1 - (K-1)\minlam/R)R}{K+1+1}$ and $\frac{(1 - (K-k)\minlam/R)R}{K+k+1}$ is decreasing in $k$. Thus, for FD $t^*_{\textrm{FD}} = \frac{(1 - \minlam/R)R}{2K}$. $\frac{\delta^*_{\textrm{HD}}}{\delta^*_{\textrm{FD}}} = \frac{t^*_{\textrm{FD}}}{t^*_{\textrm{HD}}}$.
        
        \item \textit{Case 3}: If $\frac{\minlam}{R} > \frac{1}{2K+1}$, then $\frac{(1-2\minlam/R)R}{2K} > \frac{(1 - K\minlam/R)R}{K+1} > \frac{(1 - 2(K-1)\minlam/R)R}{2K+1+1}$ and $\frac{(1 - 2(K-k)\minlam/R)R}{2K+k+1}$ is a increasing function in $k$. Thus, for half-duplex $t^*_{\textrm{HD}} = \frac{(1 - 2(K-1)\minlam/R)R}{2(K+2)}$. For FD, $\frac{(1-\minlam/R)R}{K} > \frac{(1 - (K-1)\minlam/R)R}{K+1+1} > \frac{(1 - K\minlam/R)R}{K+1}$ and $\frac{(1 - (K-k)\minlam/R)R}{K+k+1}$ is increasing in $k$. Thus, for FD $t^*_{\textrm{FD}} = \frac{(1 - K\minlam/R)R}{K+1}$. $\frac{\delta^*_{\textrm{HD}}}{\delta^*_{\textrm{FD}}} = \frac{t^*_{\textrm{FD}}}{t^*_{\textrm{HD}}}$.
    \end{itemize}
    \end{proof}
\end{lemma}

\begin{corollary}
The maximum number of hops that a linear $\cT$ can support is given by
\begin{align}
    K_{\textrm{max}} = 
    \begin{cases}
    1 + \frac{R}{2\minlam}, ~ \textrm{HD} \\
    \frac{R}{\minlam}, ~ \textrm{FD}
    \end{cases}
\end{align}

    \begin{proof}
    $t^*$ should be non-negative else \eqref{opt:delay_feas_lp_reform} is infeasible.
    \end{proof}
\end{corollary}

\begin{theorem}
If $\cT$ is linear with depth $K$. The backhaul edges have capacity $R_b$ and all the access edges have capacity $R_a$.

\begin{align}
    t^*_{\textrm{HD}} = 
     \begin{cases}
        \left[1 - \minlam\left(\frac{3}{R_b} + \frac{1}{R_a}\right)\right]\left[\frac{2K}{R_b} + \frac{K-1}{R_a}\right]^{-1}, ~ \frac{\minlam}{R} \leq \frac{R_a}{4K(R_a/R_b)^2 + (2K+1)(R_a/R_b) + 1} \\
        \left[1 - \minlam\left(\frac{2K-3}{R_b} + \frac{1}{R_a}\right)\right]\left[\frac{2K}{R_b} + \frac{2}{R_a}\right]^{-1}, ~ \frac{\minlam}{R} > \frac{R_a}{4K(R_a/R_b)^2 + (2K+1)(R_a/R_b) + 1}
    \end{cases}
\end{align}

\begin{align}
    t^*_{\textrm{FD}} = 
     \begin{cases}
        \left[1 - \minlam\left(\frac{1}{R_b} + \frac{1}{R_a}\right)\right]\left[\frac{K}{R_b} + \frac{K-1}{R_a}\right]^{-1}, ~ \frac{\minlam}{R} \leq \frac{R_a}{K(R_a/R_b)^2 + K(R_a/R_b) + 1} \\
        \left[1 - \minlam\left(\frac{K-1}{R_b} + \frac{1}{R_a}\right)\right]\left[\frac{K}{R_b} + \frac{1}{R_a}\right]^{-1}, ~ \frac{\minlam}{R} > \frac{R_a}{K(R_a/R_b)^2 + K(R_a/R_b) + 1}
    \end{cases}
\end{align}
And $\delta^* = \frac{-\log(1 - \eta)}{t^*}$.
\end{theorem}

\begin{corollary}
The maximum number of hops that a linear $\cT$ can support is given by
\begin{align}
    K_{\textrm{max}} = 
    \begin{cases}
    \frac{1}{2}\left(3 + R_b\left(\frac{1}{\minlam} - \frac{1}{R_a}\right)\right), ~ \textrm{HD} \\
    1 + R_b\left(\frac{1}{\minlam} - \frac{1}{R_a}\right), ~ \textrm{FD}
    \end{cases}
\end{align}

    \begin{proof}
    $t^*$ should be non-negative else \eqref{opt:delay_feas_lp_reform} is infeasible.
    \end{proof}
\end{corollary}
